R3D: Quantitative 3D Spatial Reasoning for Egocentric Wearables

Quantitative 3D spatial reasoning from egocentric RGB-D video is an important capability for next-generation wearable assistants. Yet existing benchmarks do not reflect the challenges of handling (1) natural egocentric video, (2) posed RGB-D video inputs, and (3) challenging quantitative 3D spatial reasoning Q&A. To fill this gap, we introduce R3D-Bench (Reasoning in 3D), a benchmark of 2,950 quantitative spatial reasoning questions across 15 types--spanning multiple-choice, distance-based, and volumetric reasoning questions--built on top of 57 egocentric video sequences from Aria Digital Twin. To set a strong baseline on this dataset, we introduce R3D, a model-agnostic spatial tool-calling framework. In contrast to existing approaches that directly embed 3D information into the model's input representation, R3D constructs a 3D scene from video using segmentation and depth-lifted object representations. It provides this information to an LLM through seven composable spatial tools. On R3D-Bench, R3D with Qwen3.6 35B-A3B outperforms all baselines $<$100B parameters, achieving 55.6% mean relative accuracy, a substantial increase over the second-best approach (CuTR+Tools, 47.7%). In the $\ge$100B parameter domain, our R3D Qwen3-VL 235B-A22B Thinking variant improves upon its base model by 7.7% absolute, achieving 57.0% accuracy and outperforming all open- and closed-source models except closed-source GPT-5.5 (59.1%), with which it remains competitive. We publicly release both R3D-Bench and our full implementation.

==> floats/fig_seg_comparison.tex <==
\begin{figure}[!t]
\centering
\setlength{\tabcolsep}{1pt}
\newcommand{\segfig}[1]{\includegraphics[width=0.22\columnwidth]{figures/seg_comparison/#1}}
\begin{tabular}{@{}m{0.4cm}m{0.22\columnwidth}m{0.22\columnwidth}m{0.22\columnwidth}m{0.22\columnwidth}@{}}
& \centering\scriptsize\textbf{coffee pod carousel} & \centering\scriptsize\textbf{wooden fork} & \centering\scriptsize\textbf{mug} & \centering\arraybackslash\scriptsize\textbf{frying pan} \\[1pt]
\rotatebox{90}{\tiny\textbf{GT}} &
\segfig{col1_gt.png} & \segfig{col2_gt.png} & \segfig{col3_gt.png} & \segfig{col4_gt.png} \\[1pt]
\rotatebox{90}{\tiny\textbf{GT Crop}} &
\segfig{col1_gt_crop.png} & \segfig{col2_gt_crop.png} & \segfig{col3_gt_crop.png} & \segfig{col4_gt_crop.png} \\[2pt]
\rotatebox{90}{\tiny\textbf{SAM3}} &
\segfig{col1_sam3.png} & \segfig{col2_sam3.png} & \segfig{col3_sam3.png} & \segfig{col4_sam3.png} \\[1pt]
\rotatebox{90}{\tiny\textbf{SAM3 Crop}} &
\segfig{col1_sam3_crop.png} & \segfig{col2_sam3_crop.png} & \segfig{col3_sam3_crop.png} & \segfig{col4_sam3_crop.png} \\
\end{tabular}
\caption{Example visual inputs in \ours{}-Bench. Rows 1--2: ground truth mask with zoomed crop. Rows 3--4: SAM3 mask with zoomed crop. Challenges: distant object with thin elements (coffee pod carousel), motion blur (wooden fork), distant object on dark surface (frying pan).}
\label{fig:seg_comparison}
\end{figure}


==> floats/tab_app_gemini_overlay.tex <==
\begin{table}[h]
\centering
\small
\caption{Gemini 3 Flash with different object overlays (all 2,950 questions, parse failures counted as wrong). \textit{SAM3 tracks} is the setting used in Table~\ref{tab:main_results}. The pointing overlays mark each referenced object only on its pointing frame, using the ground-truth pointing mask that \ours{} uses to prompt SAM3.}
\label{tab:gemini_overlay}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Overlay & MC & Distance & Volume & Overall \\
\midrule
SAM3 tracks (Table~\ref{tab:main_results}) & 77.1 & 46.1 & 27.3 & 52.7 \\
None & 78.3 & 45.8 & 30.1 & 53.5 \\
Pointing mask & \textbf{80.8} & 46.4 & \textbf{35.4} & \textbf{55.7} \\
Pointing box & 79.9 & \textbf{47.4} & 34.0 & 55.6 \\
\bottomrule
\end{tabular}
\end{table}


==> floats/tab_benchmark_comparison.tex <==
\begin{table}[t]
\centering
\caption{Comparison of spatial reasoning benchmarks. \ours{}-Bench is the only benchmark combining all properties needed for evaluating wearable spatial assistants.}
\label{tab:benchmark_comparison}
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lcccc@{}}
\toprule
 & \rotatebox{70}{Nat.\ Egocentric} & \rotatebox{70}{Video} & \rotatebox{70}{Depth+Pose} & \rotatebox{70}{Quantitative Q\&A} \\
\midrule
ScanQA              & --          & --          & --          & --          \\
SQA3D               & --          & --          & --          & --          \\
EmbodiedScan$^*$    & --          & \checkmark  & \checkmark  & --          \\
SpatialVLM          & --          & --          & --          & \checkmark  \\
SpatialRGPT-Bench   & --          & --          & --          & \checkmark  \\
CA-VQA              & --          & --          & \checkmark  & \checkmark  \\
OpenEQA             & \checkmark  & \checkmark  & --          & --          \\
VSI-Bench$^\dagger$ & --          & \checkmark  & --          & \checkmark  \\
OSI-Bench$^\ddagger$ & \checkmark  & \checkmark  & --          & \checkmark  \\
\midrule
\textbf{\ours{}-Bench} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} \\
\bottomrule
\end{tabular}

\vspace{2pt}
{\scriptsize $^*$ = detection/grounding tasks, not Q\&A; $^\dagger$ = RGB-only video from scanner walkthroughs, not natural egocentric motion; $^\ddagger$ = LiDAR used for GT generation. Depth not available as an input.}
\end{table}


==> floats/tab_cd_and_runtime.tex <==
\begin{table*}[t]
\begin{minipage}[t]{0.52\textwidth}
\centering
\caption{Chamfer distance (cm$^2$) between 3D representations and GT meshes. \colorbox{gray!15}{Gray row}: oracle using ground-truth segmentation masks.}
\label{tab:cd_comparison}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}l|rrr|rrr|rrr@{}}
\toprule
 & \multicolumn{3}{c|}{CD: Pred$\to$GT} & \multicolumn{3}{c|}{CD: GT$\to$Pred} & \multicolumn{3}{c}{CD (Full)} \\
 & P5 & P50 & P95 & P5 & P50 & P95 & P5 & P50 & P95 \\
\midrule
R3D Pointcloud    & 0.14 & 1.53 & 16.1 & 0.37 & 2.93 & 28.5 & 0.58 & 4.66 & 42.9 \\
R3D Aniso         & 0.17 & 4.46 & 175.6 & 0.19 & 2.17 & 24.8 & 0.37 & 7.59 & 198.5 \\
R3D Iso           & \textbf{0.12} & \textbf{0.89} & \textbf{14.5} & \textbf{0.15} & \textbf{0.88} & \textbf{18.2} & \textbf{0.28} & \textbf{1.86} & \textbf{30.6} \\
\rowcolor{gray!15} R3D Iso (GT Seg)  & 0.12 & 0.60 &  7.0 & 0.15 & 0.68 &  6.5 & 0.29 & 1.33 & 13.0 \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\caption{Per-question runtime comparison. CuTR+T = CuTR+Tools; S3D = SAM3D.}
\label{tab:runtime}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}l|rrrr|r|r@{}}
\toprule
 & \multicolumn{4}{c|}{Avg Preproc.\ Time (s)} & \multicolumn{1}{c|}{Model} & \multicolumn{1}{c}{Total} \\
 & SAM3 & CuTR & Lift & S3D & \multicolumn{1}{c|}{Latency (s)} & \multicolumn{1}{c}{(s)} \\
\midrule
V3D-LLM              & 52.2 & 22.0 & --- & --- &  0.8 & 75.0 \\
SRGPT                 & 52.2 & ---  & --- & --- &  3.1 & 55.3 \\
CuTR+T (8B)          & 52.2 & 22.0 & --- & --- &  2.0 & 76.2 \\
CuTR+T (35B)         & 52.2 & 22.0 & --- & --- &  5.7 & 79.9 \\
\ours{} (8B)          & 52.2 & ---  & 1.1 & 4.8 &  2.0 & 60.1 \\
\ours{} (35B)         & 52.2 & ---  & 1.1 & 4.8 &  5.7 & 63.8 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table*}

